Learning Checklists to Reduce Lottery Effects in Scientific Peer Review

Reviewer lottery error describes error due to a small set of peer reviews attending to only some of the issues with a paper that a larger pool of eligible reviewers would raise. We show this error can be reduced by surfacing a checklist of criticisms learned from a historical review corpus. Our approach generates a tree of checklists representing coarsenings of the atomic review claim space, then selects the coarsening that maximizes a theoretically-motivated measure of correlated agreement among reviewers. We realize this approach with an LLM-assisted pipeline and test it on NeurIPS 2021 and ICLR 2022 review data. In simulated review with LLM reviewers, the learned checklist reduces the mean squared error (MSE) of a three reviewer committee by 58% on NeurIPS and 21% on ICLR, and on both venues the checklist with the highest correlated agreement has the lowest error for committees of three or more. In a human study with 20 participants, the learned NeurIPS checklist lowers the MSE of a paper ranking, measured against the NeurIPS 2021 order, from 0.48 to 0.22.

==> figures/figstyle.tex <==
% Shared visual language for the TikZ figures. Input at the top of each figure file.
% Sizes assume the figure is typeset at (close to) \textwidth, so that the
% \resizebox in the caller scales by roughly 1. Every line ends in % because
% pipeline.tex is input inside a \resizebox, where stray spaces add width.
\definecolor{stA}{RGB}{62,110,168}\definecolor{stAl}{RGB}{232,240,250}%
\definecolor{stB}{RGB}{201,110,32}\definecolor{stBl}{RGB}{252,241,229}%
\definecolor{stC}{RGB}{72,150,86}\definecolor{stCl}{RGB}{230,243,232}%
\definecolor{stX}{RGB}{176,64,64}\definecolor{stXl}{RGB}{248,234,234}%
\colorlet{stPanel}{black!3}%
% Font sizes are the 10pt-class values of \footnotesize and \scriptsize; node
% widths are tuned to them, so they must not grow with an 11pt document class.
\tikzset{%
  fig title/.style={font=\fontsize{8}{9.5}\selectfont\bfseries, inner sep=0pt},
  fig head/.style={font=\fontsize{7}{8}\selectfont\bfseries, inner sep=0pt},
  fig body/.style={font=\fontsize{7}{8}\selectfont, inner sep=0pt},
  fig note/.style={font=\fontsize{7}{8}\selectfont, text=black!60, inner sep=0pt},
  fig annot/.style={font=\fontsize{6.5}{7.8}\selectfont\itshape, text=black!60, inner sep=0pt},
  fig panel/.style={rounded corners=2pt, draw=none, fill=#1},
  fig panel/.default=stPanel,
  fig card/.style={rounded corners=2pt, draw=#1!45, line width=0.5pt},
  fig arrow/.style={-{Stealth[length=3.2pt, width=2.6pt]}, line width=0.55pt, draw=black!40},
  fig span/.style={{Stealth[length=3.0pt]}-{Stealth[length=3.0pt]}, line width=0.7pt},
}%

